Look-up and Adapt: A One-shot Semantic Parser

Computing devices have recently become capable of interacting with their end users via natural language. However, they can only operate within a limited "supported" domain of discourse and fail drastically when faced with an out-of-domain utterance, mainly due to the limitations of their semantic parser. In this paper, we propose a semantic parser that generalizes to out-of-domain examples by learning a general strategy for parsing an unseen utterance through adapting the logical forms of seen utterances, instead of learning to generate a logical form from scratch. Our parser maintains a memory consisting of a representative subset of the seen utterances paired with their logical forms. Given an unseen utterance, our parser works by looking up a similar utterance from the memory and adapting its logical form until it fits the unseen utterance. Moreover, we present a data generation strategy for constructing utterance-logical form pairs from different domains. Our results show an improvement of up to 68.8% on one-shot parsing under two different evaluation settings compared to the baselines.

==> one-shot semantic parsing_arxiv/grammar_person.tex <==
\begin{table*}[t!]
\centering
\begin{tabular}{|llll|}
\hline \hline
Left-hand-side & & Source(Utterance) & Target(Logical Form)\\
\hline
\hline
\textbf{PSN} & $\to$ & john  & \texttt{(person john)}\\
\hline 
\textbf{PSN} & $\to$ & mary  & \texttt{(person mary)}\\
\hline
\textbf{PSN} & $\to$ & colleagues  & \texttt{(person colleague)}\\
\hline
\textbf{PSN} & $\to$ & professors  & \texttt{(person professor)}\\
\hline
\textbf{PSN\_REL} & $\to$ & parents & \texttt{(relation parent)}\\
\hline
\textbf{PSN\_REL} & $\to$ & children & \texttt{(relation child)}\\
\hline
\textbf{PSN\_REL} & $\to$ & hometown & \texttt{(relation hometown)}\\
\hline
\textbf{PSN\_REL} & $\to$ & salary & \texttt{(relation salary)}\\
\hline
\textbf{FIELD} & $\to$  &\textbf{PSN\_REL$_1$} of \textbf{PSN$_2$} & \texttt{(field} \textbf{PSN\_REL$_1$} \textbf{PSN$_2$}\texttt{)}\\
\hline
\textbf{FIELD} & $\to$  & \textbf{PSN$_2$} 's \textbf{PSN\_REL$_1$}  & \texttt{(field} \textbf{PSN\_REL$_1$} \textbf{PSN$_2$}\texttt{)}\\
\hline
\textbf{CMD} & $\to$  & set \textbf{FIELD$_1$} to \textbf{VALUE$_2$}  & \texttt{(set} \textbf{FIELD$_1$} \textbf{VALUE$_2$}\texttt{)}\\
\hline
\textbf{VALUE} & $\to$ & \textbf{FIELD$_1$} & \textbf{FIELD$_1$}\\
\hline
\textbf{VALUE} & $\to$ & \textbf{PSN$_1$} & \textbf{PSN$_1$}\\
\hline
\textbf{S} & $\to$ & \textbf{FIELD$_1$} & \textbf{FIELD$_1$}\\
\hline
\textbf{S} & $\to$ & \textbf{CMD$_1$} & \textbf{CMD$_1$}\\
\hline
\hline
\end{tabular}
% \begin{tablenotes}
%       \small
%       \item 
%     \end{tablenotes}
\caption{This is a selected subset of the grammar used to generate data for the \emph{person} domain. Rules not shown here include those for introducing flexibility in language and rules for additional entities and relations.}
\label{tab:person_grammar}
\end{table*}

==> one-shot semantic parsing_arxiv/grammar_restaurant.tex <==

\begin{table*}[t!]
\centering
\begin{tabular}{|llll|}
\hline \hline
Left-hand-side & & Source(Utterance) & Target(Logical Form)\\
\hline
\hline
\textbf{RST} & $\to$ & chinese restaurant  & \texttt{(restaurant chinese)}\\
\hline 
\textbf{RST} & $\to$ & italian restaurant  & \texttt{(restaurant italian)}\\
\hline
\textbf{RST} & $\to$ & french restaurant  & \texttt{(restaurant french)}\\
\hline
\textbf{RST} & $\to$ & german restaurant  & \texttt{(restaurant german)}\\
\hline
\textbf{RST\_REL} & $\to$ & address & \texttt{(relation address)}\\
\hline
\textbf{RST\_REL} & $\to$ & reviews & \texttt{(relation reviews)}\\
\hline
\textbf{RST\_REL} & $\to$ & dishes & \texttt{(relation dishes)}\\
\hline
\textbf{RST\_REL} & $\to$ & price & \texttt{(relation price)}\\
\hline
\textbf{FIELD} & $\to$  &\textbf{RST\_REL$_1$} of \textbf{RST$_2$} & \texttt{(field} \textbf{RST\_REL$_1$} \textbf{RST$_2$}\texttt{)}\\
\hline
\textbf{FIELD} & $\to$  & \textbf{PSN$_2$} 's \textbf{RST\_REL$_1$}  & \texttt{(field} \textbf{RST\_REL$_1$} \textbf{RST$_2$}\texttt{)}\\
\hline
\textbf{CMD} & $\to$  & set \textbf{FIELD$_1$} to \textbf{VALUE$_2$}  & \texttt{(set} \textbf{FIELD$_1$} \textbf{VALUE$_2$}\texttt{)}\\
\hline
\textbf{VALUE} & $\to$ & \textbf{FIELD$_1$} & \textbf{FIELD$_1$}\\
\hline
\textbf{VALUE} & $\to$ & \textbf{RST$_1$} & \textbf{RST$_1$}\\
\hline
\textbf{S} & $\to$ & \textbf{FIELD$_1$} & \textbf{FIELD$_1$}\\
\hline
\textbf{S} & $\to$ & \textbf{CMD$_1$} & \textbf{CMD$_1$}\\
\hline
\hline
\end{tabular}
% \begin{tablenotes}
%       \small
%       \item 
%     \end{tablenotes}
\caption{This is a selected subset of the grammar used to generate data for the \emph{restaurant} domain. Rules not shown here include those for introducing flexibility in language and rules for additional entities and relations.}
\label{tab:restaurant_grammar}
\end{table*}

==> one-shot semantic parsing_arxiv/table_dataset_examples.tex <==
\begin{table*}[h]
\centering 
\resizebox{1.8\columnwidth}{!}{%
\begin{tabular}{|cll|}
\hline \hline
& Domain & Utterance \& Logical Form\\
\hline \hline
$a_1$&\emph{person}& the hometown field of john \\
&& (field (relation hometown) (person john))\\
$a_2$&\emph{person}& set her 's parents with classmates \\
&& (set (field (relation parent) (person reference)) (person classmate))\\
\hline
$b_1$&\emph{restaurant}& irish restaurant instances 's price field \\
&& (field (relation price) (restaurant irish))\\
$b_2$&\emph{restaurant}& set address field of all irish restaurant as indian restaurant 's price
 \\
&& (set (field (relation address) (restaurant irish)) (field (relation price) (restaurant indian)))\\
\hline
$c_1$&\emph{event}& the start time of lectures\\
&& (field (relation start) (event lecture)) \\
$c_2$&\emph{event}& set the attendants of that event to organizers field of receptions instances
 \\
&& (set (field (relation attendant) (event reference)) (field (relation organizer) (event reception)))\\
\hline
$d_1$&\emph{course}& size of my history course instances \\
&& (field (relation size) (course history))\\
$d_2$&\emph{course}& set all history course instances 's prerequisite field as physics course
\\
&& (set (field (relation prerequisite) (course history)) (course physics))\\
\hline
$e_1$&\emph{animal}& life span of all lion instances\\
&&(field (relation span) (animal lion))\\
$e_2$&\emph{animal}& set fish instances 's family field with dog \\
&& 
(set (field (relation family) (animal fish)) (animal dog))\\
\hline
$f_1$&\emph{vehicle}& the source field of all buses
 \\
&& (field (relation source) (vehicle bus))\\
$f_2$&\emph{vehicle} & set operators of all subways as buses instances \\
&& (set (field (relation operator) (vehicle subway)) (vehicle bus))\\
\hline
\hline
\end{tabular}
}
% \begin{tablenotes}
%       \small
%       \item 
%     \end{tablenotes}
\caption{Sample utterance-logical form pairs from each domain of discourse. Sentences $a_1$ ... $f_1$ parse to commands that retrieve a field of an object. Sentences $a_2$ ... $f_2$ parse to commands which set a field of an object to a constant or a field of another object. The grammar we use do not constrain the type of the set command. As a consequence, some sentences generated are not semantically correct according to a human interpreter but still they preserve the sentence structure. Sentence $b_2$, $e_2$, and $f_2$ are examples of this phenomena.}
\label{tab:dataset_examples}
\end{table*}

==> one-shot semantic parsing_arxiv/table_datastats.tex <==
\begin{table*}[t!]
\small
\centering
\begin{tabular}{cc|c|c|c|c|c|c|}
\cline{3-8}
& & \multicolumn{6}{|c|}{\textbf{domain of discourse}}\\
\cline{3-8}
& & person & restaurant & event & course & animal & vehicle\\
\hline
\multicolumn{1}{ |c  }{\multirow{3}{*}{$D_{old}$}}
    & full  & 737   & 810   & 911   &  960  & 801  & 729\\
\multicolumn{1}{ |c  }{}  
    & d=2   & 417   & 490   & 591   & 640   & 481  & 409\\
\multicolumn{1}{ |c  }{}  
    & d=3   & 320   & 320   & 320   & 320   & 320  & 320\\
\hline
\multicolumn{1}{ |c  }{\multirow{3}{*}{$E_{olddev}$}}
    & full  & 96    & 96    & 96    & 96    & 96    & 96\\
\multicolumn{1}{ |c  }{}  
    & d=2   & 65    & 68    & 67    & 66    & 61    & 64\\
\multicolumn{1}{ |c  }{}  
    & d=3   & 31    & 28    & 29    & 30    & 35    & 32\\
\hline
\multicolumn{1}{ |c  }{\multirow{3}{*}{$E_{oldtest}$}}
    & full  & 96    & 96    & 96    & 96    & 96    & 96\\
\multicolumn{1}{ |c  }{}  
    & d=2   & 63    & 60    & 61    & 62    & 67    & 64\\
\multicolumn{1}{ |c  }{}  
    & d=3   & 33    & 36    & 35    & 34    & 29    & 32\\
\hline
\multicolumn{1}{ |c  }{\multirow{3}{*}{$E_{newdev}$}}
    & full  & 96    & 96    & 96   & 96    & 96    & 96\\
\multicolumn{1}{ |c  }{}  
    & d=2   & 68    & 67    & 58   & 68    & 60    & 66\\
\multicolumn{1}{ |c  }{}  
    & d=3   & 28    & 29    & 38   & 28    & 36    & 30\\
\hline
\multicolumn{1}{ |c  }{\multirow{3}{*}{$E_{newtest}$}}
    & full  & 96    & 96    & 96    & 96   & 96   & 96\\
\multicolumn{1}{ |c  }{}  
    & d=2   & 60    & 61    & 70    & 60   & 68   & 62\\
\multicolumn{1}{ |c  }{}  
    & d=3   & 36    & 35    & 26    & 36   & 28   & 34\\
\hline
\multicolumn{1}{ |c  }{\multirow{3}{*}{$M_{old}$}}
    & full  & 23    & 16    & 16    & 16    & 16    & 15\\
\multicolumn{1}{ |c  }{}  
    & d=1   & 20    & 13    & 13    & 13    & 13    & 12\\
\multicolumn{1}{ |c  }{}  
    & d=2   & 2     & 2     & 2     & 2     & 2     & 2\\
\multicolumn{1}{ |c  }{}  
    & d=3   & 1     & 1     & 1     & 1     & 1     & 1\\
\hline
\multicolumn{1}{ |c  }{\multirow{3}{*}{$M_{new}$}}
    & full  & 27    & 20    & 20    & 20    & 20    & 19\\
\multicolumn{1}{ |c  }{}  
    & d=1   & 24    & 17    & 17    & 17    & 17    & 16\\
\multicolumn{1}{ |c  }{}  
    & d=2   & 2     & 2     & 2     & 2     & 2     & 2\\
\multicolumn{1}{ |c  }{}  
    & d=3   & 1     & 1     & 1     & 1     & 1     & 1\\
\hline
\end{tabular}
% \begin{tablenotes}
% 	\item
% \end{tablenotes}
\caption{Dataset Statistics: sizes of each component with depth breakdown. Please refer to \S~\ref{sec:dataset_generation} for the precise definition of each row of the table. In the \emph{extension} scenario, for each domain of discourse $d$, the model is trained on examples from $D_{old,d}$ using $M_{old,d}$ as memory and is evaluated on examples from $E_{newdev,d}$ and $E_{newtest,d}$ using $M_{new,d}$ as memory. In the \emph{transfer} scenario, for each domain of discourse $d$, the model is trained on $\cup_{d'\neq d} D_{old,d'}$ using $\cup_{d'\neq d} M_{old,d'}$ as memory, and is evaluated on $E_{olddev,d}$ and $E_{oldtest,d}$ using $\cup_{\forall d'} M_{old,d'}$ as memory.}
\label{tab:dataStats}
\end{table*}

==> one-shot semantic parsing_arxiv/table_domain_of_sample_scfg.tex <==
\begin{table}[h]
\centering \small
\begin{tabular}{|ll|}
\hline \hline
Utterance & Logical Form\\
\hline \hline
John & \texttt{john}\\
\hline
Mary & \texttt{mary}\\
\hline
 parents & \texttt{parent}\\
\hline
 children & \texttt{child}\\
\hline
 parents of John & \texttt{(field parent john)}\\
\hline
 parents of Mary & \texttt{(field parent mary)}\\
\hline
 children of John & \texttt{(field child john)}\\
\hline
 children of Mary & \texttt{(field child mary)}\\
\hline
 John 's parents& \texttt{(field parent john)}\\
\hline
 Mary 's parents & \texttt{(field parent mary)}\\
\hline
 John 's children& \texttt{(field child john)}\\
\hline
 Mary 's children & \texttt{(field child mary)}\\
\hline
\hline
\end{tabular}
% \begin{tablenotes}
%       \small
%       \item 
%     \end{tablenotes}
\caption{Domain of the sample SCFG $G_{sample}$. The rules of this SCFG are presented in the Appendix \ref{sec:rules}. The domain of the sample SCFG is the set of all $\langle$source, \texttt{target}$\rangle$ pairs listed in this table.}
\label{tab:example_domain}
\end{table}

==> one-shot semantic parsing_arxiv/table_extension.tex <==
\begin{table*}[h]
\centering \small
\resizebox{1.5\columnwidth}{!}{%
\begin{tabular}{cc|c|c|c|c|c|c|}
\cline{3-8}
& & \multicolumn{6}{|c|}{\textbf{extension}}\\
\cline{3-8}
& & person & restaurant & event & course & animal & vehicle\\
\hline
\multicolumn{1}{|c}{\multirow{3}{*}{Sequence-To-Sequence}}
    & full & 20.1 & 25.1 & 26.1&  19.9 & 25.0 & 18.8\\
\multicolumn{1}{ |c  }{}  
    & d=2& 25.0& 18.1 & 20.0& 31.8& 26.5& 25.9\\
\multicolumn{1}{ |c  }{}  
    & d=3& 13.9& 37.3& 42.4& 0.0& 21.5& 5.8\\
\hline
\multicolumn{1}{|c}{\multirow{3}{*}{LOOKUPADAPT}}
    & full & \bf 45.9 & \bf 61.7 & \bf 85.5 & \bf 79.2& \bf 63.6& \bf 87.6\\
\multicolumn{1}{ |c  }{}  
    & d=2& 56.7& 85.4& 94.5& 86.7& 70.1& 93.6\\
\multicolumn{1}{ |c  }{}  
    & d=3& 27.8& 20.0& 61.7&  66.7&  46.5&  76.5\\
\hline
\end{tabular}
}
\caption{Test Accuracy on the \textbf{extension} Dataset.}
\label{tab:results-extension}
\end{table*}


==> one-shot semantic parsing_arxiv/table_sample_scfg.tex <==
\begin{table*}[t!]
\centering
\begin{tabular}{|llll|}
\hline \hline
Left-hand-side & & Source(Utterance) & Target(Logical Form)\\
\hline
\hline
\textbf{PSN} & $\to$ & John  & \texttt{john}\\
\hline 
\textbf{PSN} & $\to$ & Mary  & \texttt{mary}\\
\hline
\textbf{PSN\_REL} & $\to$ & parents & \texttt{parent}\\
\hline
\textbf{PSN\_REL} & $\to$ & children & \texttt{child}\\
\hline
\textbf{FIELD} & $\to$  &\textbf{PSN\_REL$_1$} of \textbf{PSN$_2$} & \texttt{(field} \textbf{PSN\_REL$_1$} \textbf{PSN$_2$}\texttt{)}\\
\hline
\textbf{FIELD} & $\to$  & \textbf{PSN$_2$} 's \textbf{PSN\_REL$_1$}  & \texttt{(field} \textbf{PSN\_REL$_1$} \textbf{PSN$_2$}\texttt{)}\\
\hline
\textbf{S} & $\to$ & \textbf{PSN$_1$} & \textbf{PSN$_1$}\\
\hline 
\textbf{S} & $\to$ & \textbf{PSN\_REL$_1$} & \textbf{PSN\_REL$_1$}\\
\hline 
\textbf{S} & $\to$ & \textbf{FIELD$_1$} & \textbf{FIELD$_1$}\\
\hline
\hline
\end{tabular}
% \begin{tablenotes}
%    \small
%    \item 
% \end{tablenotes}
\caption{Sample SCFG $G_{sample}$. The subscripts indicate linking of terminals/nonterminals in source and target. A SCFG rule can only be applied to linked terminals/nonterminals together.}
\label{tab:example_scfg_person}
\end{table*}

==> one-shot semantic parsing_arxiv/table_sample_trace_of_algo.tex <==
\begin{table*}[h!]
\centering
\footnotesize
\begin{tabular}{|@{\hskip2pt}l@{\hskip3pt}|@{\hskip3pt}l@{\hskip3pt}|@{\hskip3pt}c@{\hskip3pt}|@{\hskip3pt}c@{\hskip2pt}|}
\hline \hline
 Func & Description  &
 \shortstack{New utterance and\\
            current logical form } &
 Memory\\
\hline \hline

    \textsc{LkUpNAdpt}&
    \shortstack[l]{Initial call always has\\
                    uniform attention.} &
    \shortstack{\textbf{[John 's parents]}\\
                None} &
    \shortstack{$\langle$John, \texttt{john}$\rangle$\\ 
                $\langle$Mary, \texttt{mary}$\rangle$\\
                $\langle$Mary 's parents ,\texttt{(field parent mary)}$\rangle$}\\
\hline
    \textsc{LookUp}&
    \shortstack[l]{Retrieves entry $\star$ from\\
                    memory by utterance\\
                    similarity.} &
    \shortstack{\textbf{[John 's parents]}\\
                \texttt{(field parent mary)}} &
    \shortstack{$\langle$John, \texttt{john}$\rangle$\\ 
                $\langle$Mary, \texttt{mary}$\rangle$\\
                $\star$ $\langle$Mary 's parents ,\texttt{(field parent mary)}$\rangle$}\\
\hline
    ::\textsc{Adapt}&
    \shortstack[l]{Adapt first child.\\
            \texttt{parent} is aligned to\\
            \textbf{parents}. YES, they\\
            match, keep \texttt{parent}.\\
            There's no children. \\
            Return.} &
    \shortstack{John 's \textbf{[parents]}\\
                \texttt{(field [parent] mary)}} &
    \shortstack{$\langle$John, \texttt{john}$\rangle$\\ 
                $\langle$Mary, \texttt{mary}$\rangle$\\
                 $\langle$Mary 's parents ,\texttt{(field parent mary)}$\rangle$}\\
\hline
    ::\textsc{Adapt}&
    \shortstack[l]{Adapt second child.\\
            \texttt{mary} is aligned to\\
            \textbf{John}. NO, they\\
            don't match.\\
            Find replacement and\\
            return it.} &
    \shortstack{\textbf{[John]} 's parents\\
                \texttt{(field parent [mary])}} &
    \shortstack{$\langle$John, \texttt{john}$\rangle$\\ 
                $\langle$Mary, \texttt{mary}$\rangle$\\
                 $\langle$Mary 's parents ,\texttt{(field parent mary)}$\rangle$}\\
\hline
    ::::\textsc{LkUpNAdpt}&
    \shortstack[l]{Find replacement\\
                    for \texttt{mary}.} &
    \shortstack{\textbf{[John]} 's parents\\
                \texttt{(field parent mary)}} &
    \shortstack{$\langle$John, \texttt{john}$\rangle$\\ 
                $\langle$Mary, \texttt{mary}$\rangle$\\
                $\langle$Mary 's parents ,\texttt{(field parent mary)}$\rangle$}\\
\hline
    ::::\textsc{LookUp}&
    \shortstack[l]{Retrieves entry $\star$ from\\
                    memory by utterance\\
                    similarity.} &
    \shortstack{\textbf{[John]} 's parents\\
                \texttt{(field parent mary)}} &
    \shortstack{$\star$ $\langle$John, \texttt{john}$\rangle$\\ 
                $\langle$Mary, \texttt{mary}$\rangle$\\
                $\langle$Mary 's parents ,\texttt{(field parent mary)}$\rangle$}\\
\hline
    ::::\textsc{LkUpNAdpt}&
    \shortstack[l]{There's no children. \\
                Return \texttt{john}} &
    \shortstack{\textbf{[John]} 's parents\\
                \texttt{(field parent mary)}} &
    \shortstack{$\langle$John, \texttt{john}$\rangle$\\ 
                $\langle$Mary, \texttt{mary}$\rangle$\\
                $\langle$Mary 's parents ,\texttt{(field parent mary)}$\rangle$}\\
\hline
    \textsc{LkUpNAdpt}&
    \shortstack[l]{Replace \texttt{mary} with\\
                   \texttt{john}. Exhausted\\
                   all children, return\\
                   the current logical \\
                   form.} &
    \shortstack{\textbf{[John 's parents]}\\
                \texttt{(field parent john)}} &
    \shortstack{$\langle$John, \texttt{john}$\rangle$\\ 
                $\langle$Mary, \texttt{mary}$\rangle$\\
                $\langle$Mary 's parents ,\texttt{(field parent mary)}$\rangle$}\\
\hline
\hline
\end{tabular}
% \begin{tablenotes}
% 	\item 
% \end{tablenotes}
\caption{Trace of a sample run of the algorithm with sample memory, utterance, and attention. The attention weights (argument $\bm{w}'$ to \textsc{LookUpAndAdapt} and variable $\bm{w}$ in \textsc{Adapt}) are visualized as brackets. Bracketed words in the \emph{utterance} receive more attention, un-bracketed words receive less attention. For \textsc{Adapt} calls, bracketed words in the \emph{logical form} indicate the current subtree of the whole logical form tree that the algorithm is looking at (the argument \texttt{T} to \textsc{Adapt}). Colons are used to indicate the depth of the call stack.}
\label{tab:trace}
\end{table*}

==> one-shot semantic parsing_arxiv/table_transfer.tex <==
\begin{table*}[h]
\centering \small
\resizebox{1.5\columnwidth}{!}{%
\begin{tabular}{cc|c|c|c|c|c|c|}
 \cline{3-8}
 & & \multicolumn{6}{|c|}{\textbf{transfer}}\\
 \cline{3-8}
 & & person & restaurant & event & course & animal & vehicle\\
 \hline
\multicolumn{1}{|c}{\multirow{3}{*}{Sequence-To-Sequence}}
    & full &  5.2 & 29.2 & 5.2&  \bf 19.9 & \bf 35.5& \bf 12.5\\
\multicolumn{1}{ |c  }{}  
    & d=2& 6.4&  41.7& 4.9&  27.5&  44.9& 15.6\\
\multicolumn{1}{ |c  }{}  
    & d=3& 3.1&  8.4&  5.7&  6.0& 13.8& 6.3\\
 \hline
\multicolumn{1}{|c}{\multirow{3}{*}{LOOKUPADAPT}}
    & full &  \bf 41.8& \bf  43.8&  \bf 8.4&  16.7&  28.3&  11.5\\
\multicolumn{1}{ |c  }{}  
    & d=2&  52.5& 53.4&  13.2&  24.2&  37.3&  14.1\\
\multicolumn{1}{ |c  }{}  
    & d=3&  21.4&  27.8& 0.0&  3.0&  6.9&  6.3\\
\hline \hline
\multicolumn{1}{|c}{\multirow{3}{*}{ORACLE-DISCRIM}}
    & full  &  46.9 &   45.8& 12.5  & 29.2&  33.3&  25.0\\
\multicolumn{1}{ |c  }{}  
    & d=2   & 55.6  &   56.7& 18.0  & 41.8&  44.8& 29.7\\
\multicolumn{1}{ |c  }{}  
    & d=3   & 30.3  &  27.8 & 2.9   &  5.9&  6.9&  15.6\\
\hline
\multicolumn{1}{|c}{\multirow{3}{*}{PRETRAIN-ENC}}
    & full  & 98.0& 100.0& 100.0& 99.0&  100.0&96.9\\
\multicolumn{1}{ |c  }{}  
    & d=2 & 100.0& 100.0& 100.0& 100.0& 100.0&  100.0\\
\multicolumn{1}{ |c  }{}  
    & d=3 & 94.0& 100.0& 100.0& 97.1& 100.0& 90.1\\
\hline
\end{tabular}
}
\caption{Test Accuracy on the \textbf{transfer} Dataset.}
\label{tab:results-transfer}
\end{table*}
